Reducing False Positives in Static Bug Detection with LLMs: An Empirical Study in Industry

Static analysis tools (SATs) are widely adopted in both academia and industry for improving software quality, yet their practical use is often hindered by high false positive rates, especially in large-scale enterprise systems. These false alarms demand substantial manual inspection, creating severe inefficiencies in industrial code review. While recent work has demonstrated the potential of large language models (LLMs) for false alarm reduction on open-source benchmarks, their effectiveness in real-world enterprise settings remains unclear. To bridge this gap, we conduct the first comprehensive empirical study of diverse LLM-based false alarm reduction techniques in an industrial context at Tencent, one of the largest IT companies in China. Using data from Tencent's enterprise-customized SAT on its large-scale Advertising and Marketing Services software, we construct a dataset of 433 alarms (328 false positives, 105 true positives) covering three common bug types. Through interviewing developers and analyzing the data, our results highlight the prevalence of false positives, which wastes substantial manual effort (e.g., 10-20 minutes of manual inspection per alarm). Meanwhile, our results show the huge potential of LLMs for reducing false alarms in industrial settings (e.g., hybrid techniques of LLM and static analysis eliminate 94-98% of false positives with high recall). Furthermore, LLM-based techniques are cost-effective, with per-alarm costs as low as 2.1-109.5 seconds and $0.0011-$0.12, representing orders-of-magnitude savings compared to manual review. Finally, our case analysis further identifies key limitations of LLM-based false alarm reduction in industrial settings.

==> section/evaluation/rq2.tex <==
\subsection{RQ2: Effectiveness of traditional learning based vulnerability detection methods}
\label{sec:rq2_result}

Table~\ref{table:rq2} presents the results of four representative deep learning–based vulnerability detection methods on our dataset.

\input{table/rq2_result}



\parabf{Overall Performance.} Overall, the performance of these methods is unsatisfactory, with the highest accuracy reaching only from 0.36 to 0.44 (except for LineVul). Two key factors may account for this limitation. First, deep learning–based methods are highly dependent on training data distribution. These learning-based models trained on existing benchmark datasets perform poorly when directly applied to previously unseen enterprise code, where large-scale, labeled training data is scarce. This lack of sufficient domain-specific training data makes fine-tuning such models for enterprise use particularly challenging.
Second, prior studies~\cite{du2024vul} have shown that learning-based approaches often struggle to capture the true root causes of bugs. Instead, they tend to rely on superficial statistical patterns or secondary code features correlated with buggy functions. As a result, these methods are inherently limited in their ability to generalize to real-world enterprise bug detection.


\parabf{Methods Comparison.} Although Linevul reports a seemingly high accuracy of 0.76, this result stems from its tendency to classify all warnings as false positives. Since our dataset contains a large proportion of false positive cases, this bias inflates its accuracy but undermines practical value. A likely reason is that LineVul was trained on the highly imbalanced BigVul dataset, where most samples are non-vulnerable. By contrast, the other methods all achieve accuracies below 0.44. Among them, ReGVD stands out due to its comparatively high recall of 0.87. However, its false positive recall is only 0.19, meaning that it only successfully eliminates 19\% of false positives. This limited effectiveness in reducing false alarms still imposes substantial manual validation costs, restricting its overall practical benefit.

\parabf{Interpretability.} Traditional learning-based methods inherently suffer from poor interpretability. Their outputs are limited to predicted labels without any explanatory context, which increases the burden of manual validation during enterprise code review.

\vspace{2mm}
\begin{mdframed}[linecolor=gray,roundcorner=12pt,backgroundcolor=gray!15,linewidth=3pt,innerleftmargin=2pt, leftmargin=0cm,rightmargin=0cm,topline=false,bottomline=false,rightline = false]
\textbf{Answer to RQ2:} Due to the lack of large-scale, high-quality enterprise training data, traditional learning-based vulnerability detection methods exhibit poor performance on enterprise datasets. Moreover, their label-only predictions without interpretability further complicate subsequent manual validation. These factors collectively limit the practicality of such methods for reducing false positives in enterprise static analysis.
\end{mdframed}
% \vspace{2mm}

==> section/evaluation/rq5.tex <==
\subsection{RQ5: Bad Case Analysis}
\label{sec:rq5_result}

To better understand the limitations of LLMs in reducing false positives, we conducted a manual analysis of two types of failure cases: (1) cases where different prompt strategies failed to help LLMs distinguish between false positives and real bugs, and (2) cases where all methods failed to classify correctly. Although confidentiality constraints prevent us from presenting the actual code examples, our analysis reveals several key limitations of LLMs in bug detection.


\parabf{Limited capacity for long-context reasoning.} We observed that LLMs are significantly less effective at mitigating false positives in cases involving long code contexts. For cases where all methods failed, the average length of the function containing the warning was 95.6 lines longer than the overall dataset average, and 67.7 lines longer than cases only correctly classified by LLM4PFA but missed by other LLM-based methods. This demonstrates that LLMs struggle with extended context reasoning. Although LLM4PFA partially alleviates this issue, the limitation persists.


\parabf{Difficulty with complex cascaded constraints.} When analyzing code containing numerous loops, deeply nested conditional branches, or intricate logical expressions, LLMs often overlook boundary conditions or introduce logical inconsistencies. As a result, they fail to accurately track variable states across multiple reasoning steps. For the cases misclassified by all methods, the average number of conditional statements was 21 higher than the overall dataset average, and 18.9 higher than the subset solvable by LLM4PFA alone. This gap highlights the intrinsic weakness of LLMs in handling multi-step, complex cascaded constraints reasoning.

\parabf{Insufficient semantic understanding.} LLMs also struggle with less common syntactic constructs, pointer manipulations, and user-defined, deeply nested data structures. Their training often lacks sufficient exposure to such patterns, leading to misinterpretation and erroneous reasoning when analyzing these cases.



\vspace{2mm}
\begin{mdframed}[linecolor=gray,roundcorner=12pt,backgroundcolor=gray!15,linewidth=3pt,innerleftmargin=2pt, leftmargin=0cm,rightmargin=0cm,topline=false,bottomline=false,rightline = false]
\textbf{Answer to RQ5:}
Although LLMs demonstrate promise in reducing false positives, they still face fundamental limitations in enterprise-scale bug detection. Specifically, LLMs exhibit (1) limited effectiveness on handling long code contexts, (2) difficulty reasoning complex cascaded constraints, and (3) insufficient semantic understanding. 
These challenges remain critical directions for advancing the practical effectiveness of LLMs in future work.
\end{mdframed}



==> section/motivation.tex <==
\section{Motivating Examples}

This section presents two examples to demonstrate the limitations of traditional symbolic execution methods and existing LLM-based approaches in detecting false positives for null pointer dereference (NPD) vulnerabilities. Both examples are false positives identified by CodeQL in Linux kernel.

\input{picture/motivating_examples}

\parabf{Complex Path Constraint Reasoning}
Figure~\ref{fig:example2} presents a false positive caused by CodeQL's inability to perform precise path-sensitive analysis. In this example, a path condition ``\textit{connected \&\& md}'' (line 102) ensure the unreachability of the sink. As shown in the green-highlighted statements, when \textit{md} is \textit{true} (line 36), the target pointer \textit{tun\_info} is guaranteed to be non-null (line 34).

Beyond the green-highlighted sections, this case also involves numerous additional conditional branches (highlighted in orange), with some omitted due to space limits. Moreover, Real-world software projects present even greater complexity, featuring deeply nested loops and intricate conditional branches. Such complexity significantly reduces the effectiveness of LLM-based methods, as LLMs have limited capabilities in handling long contexts and understanding complex control and data flow in code~\cite{}.

% To address this, our framework decomposes the function level reachability analysis task into iterative, focused reasoning on specific path conditions. It  enhances the reasoning performance of LLM by narrowing its focus to specific, well-defined tasks.

\parabf{Complex Context Analysis.}
Figure~\ref{fig:example1} illustrates a false positive caused by CodeQL’s inability to perform precise context-sensitive analysis. In the second function of the function call trace from the source to the sink,  \textit{consume\_skb} performs a null check on the target pointer \textit{skb}. When \textit{skb} is null, the called function \textit{skb\_unref} returns \textit{false}, causing the program to exit via rather than propagating the value to the sink.

When analyzing the context of this case, Beyond the source-to-sink function call trace (with later functions omitted), functions in the trace involves additional contextual function calls, resulting in deeper layers of contextual information. Due to the complexity of the Linux kernel, this analysis requires handling not only function calls but also macro definitions and built-in GCC compiler functions, posing significant challenges for traditional symbolic execution.
More importantly, Figure~\ref{fig:example1} only expands the minimal contextual information (highlighted in green) necessary for manual inspection to determine the root cause of the false positive. However, existing LLM-based approaches would also consider other contextual calls (highlighted in orange), further increasing the complexity of context-sensitive analysis.


==> table/bad_case.tex <==

\begin{table}[htb]
	\centering
	% \vspace{-2mm}
    \caption{FN/FP analysis in CWE-119}
    \label{table:rq4}
    \footnotesize
    % \vspace{-2mm}
    % \textbf{}	
    \begin{adjustbox}{width=0.95\linewidth}
    \begin{tabular}{m{0.5cm}<{\centering}|m{5cm}<{\raggedright}|m{1cm}<{\centering}} \hline
    \textbf{Type} & \textbf{Reason} & \textbf{Number} \\  \hline
    \multirow{2}{*}{FN} & Inaccurate vulnerability knowledge descriptions. & 5 \\ \cline{2-3}
    & Unretrieved relevant vulnerability knowledge. & 2 \\ \cline{2-3}
    & Non-existent relevant vulnerability knowledge. & 12 \\ \cline{2-3} \hline 
    \multirow{2}{*}{FP} & Mismatched fixing solutions. & 11 \\ \cline{2-3}
    & Irrelevant vulnerability knowledge retrieval & 10 \\ \hline 
    \end{tabular}
    \end{adjustbox}
\end{table}

==> table/cwe_statistics.tex <==
\begin{table*}[htb]
	%\scriptsize
    \centering
	%\vspace{-5mm}
    \caption{The Statistics of the 10 Most Frequent CWEs}	 
    \label{table:cwe}
    \footnotesize
    \begin{adjustbox}{width=1\textwidth}
    \begin{tabular}{|p{4cm}<{\centering}|p{1cm}<{\centering}|p{1.2cm}<{\centering}|p{10cm}<{\raggedright}|} \hline
	
    \textbf{CWE ID \& Name}  & \textbf{CVE Num.}  & \textbf{Fun. Pair Num.}  & \textbf{CWE Description} \\  \hline
    CWE-416: Use After Free & 341 & 856 & Referencing memory after it has been freed can cause a program to crash, use unexpected values, or execute code. \\  \hline
    CWE-476: NULL Pointer Dereference & 196 & 353 & A NULL pointer dereference occurs when the application dereferences a pointer that it expects to be valid, but is NULL, typically causing a crash or exit. \\  \hline
    CWE-362: Concurrent Execution using Shared Resource with Improper Synchronization  & 170 & 402 & The product contains a code sequence that can run concurrently with other code, and the code sequence requires temporary, exclusive access to a shared resource, but a timing window exists in which the shared resource can be modified by another code sequence that is operating concurrently. \\  \hline
    CWE-119: Improper Restriction of Operations within the Bounds of a Memory Buffer & 130 & 217 & The product performs operations on a memory buffer, but it can read from or write to a memory location that is outside of the intended boundary of the buffer. \\  \hline
    CWE-787: Out-of-bounds Write & 124 & 235 & The product writes data past the end, or before the beginning, of the intended buffer. \\  \hline
    CWE-200: Exposure of Sensitive Information to an Unauthorized Actor & 116 & 208 & The product exposes sensitive information to an actor that is not explicitly authorized to have access to that information. \\  \hline
    CWE-125: Out-of-bounds Read & 106 & 177 & The product reads data past the end, or before the beginning, of the intended buffer. \\  \hline
    CWE-20: Improper Input Validation & 96 & 283 & The product receives input or data, but it does not validate or incorrectly validates that the input has the properties that are required to process the data safely and correctly. \\  \hline
    CWE-401: Missing Release of Memory after Effective Lifetime & 94 & 128 & The product does not sufficiently track and release allocated memory after it has been used, which slowly consumes remaining memory. \\  \hline
    CWE-190: Integer Overflow or Wraparound & 46 & 64 & The product performs a calculation that can produce an integer overflow or wraparound, when the logic assumes that the resulting value will always be larger than the original value. This can introduce other weaknesses when the calculation is used for resource management or execution control. \\  \hline
    \end{tabular}
    \end{adjustbox}
    % \vspace{-1mm}
\end{table*}

==> table/rq4_result.tex <==
\begin{table}[htb]
    \centering
    \caption{Ablation of \app{}}\label{table:rq4}
    \footnotesize
    \begin{adjustbox}{width=1\linewidth}
        \begin{tabular}{c|c|c|c|c|c|c}
        \hline
        
        \textbf{Project} &\textbf{Tech.} & \textbf{Acc.} &
        \textbf{FPR\_P} & \textbf{FPR\_R} &
        \textbf{Pre.} & \textbf{Recall} \\ \hline
        \multirow{4}{*}{Kernel}
        & \app{} & \textbf{0.9}  & \textbf{0.96} & \textbf{0.90} & \textbf{0.8} & 0.90  \\
        & \appva{} & 0.44  & 0.8  & 0.25 & 0.35 & 0.86  \\
        & \appvb{} & 0.56 & 0.95 & 0.38 & 0.41 & \textbf{0.95} \\
        & \appvc{} & 0.37 & 0.83 & 0.10 & 0.33 & \textbf{0.95} 
        \\\hline 

        \multirow{4}{*}{Openssl}
        & \app{} & \textbf{0.8}  & 0.97 & \textbf{0.78} & \textbf{0.47} & 0.89  \\
        & \appva{} & 0.46  & 0.89  & 0.40 & 0.22 & 0.78  \\
        & \appvb{} & 0.44 & 0.93 & 0.34 & 0.23 & 0.89 \\
        & \appvc{} & 0.26 & \textbf{1.0} & 0.10 & 0.20 & \textbf{1.0} 
        \\\hline 

        \multirow{4}{*}{Libav}
        & \app{} & \textbf{0.51}  & \textbf{1.0} & \textbf{0.49} & \textbf{0.07} & \textbf{1.0 } \\
        & \appva{} & 0.21  & \textbf{1.0 } & 0.18 & 0.04 & \textbf{1.0 } \\
        & \appvb{} & 0.23 & \textbf{1.0} & 0.20 & 0.04 & \textbf{1.0} \\
        & \appvc{} & 0.25 & \textbf{1.0} & 0.22 & 0.04 & \textbf{1.0} 
        \\\hline         

        
        \multirow{4}{*}{Total}
        & \app{} & \textbf{0.75} & \textbf{0.97}&\textbf{0.71} &\textbf{0.42}  & 0.91 \\
        & \appva{} & 0.37  & 0.88 & 0.26 & 0.21 &0.85 \\
        & \appvb{} &  0.42& 0.96 & 0.30 & 0.23 & 0.94 \\
        & \appvc{} & 0.29 & 0.92 & 0.14 & 0.16 & \textbf{0.97} 
        \\\hline        

        \end{tabular}
    \end{adjustbox}
\end{table}




==> table/runtime.tex <==
\begin{table}[htb]
    \centering
    \caption{Ablation of \app{}}\label{table:rq5}
    \footnotesize
    \begin{adjustbox}{width=0.8\linewidth}
        \begin{tabular}{c|c|c|c}
\hline
\textbf{Technique} & \textbf{\app{}} & \textbf{LLMSA} & \textbf{LLMDFA} \\
\textbf{Ave. Runtime} & 28.9s & 6.8s & 8.6s 
        \\\hline        
\end{tabular}
\end{adjustbox}
\end{table}

